Two Local Models for Neural Constituent Parsing

Non-local features have been exploited by syntactic parsers for capturing dependencies between sub output structures. Such features have been a key to the success of state-of-the-art statistical parsers. With the rise of deep learning, however, it has been shown that local output decisions can give highly competitive accuracies, thanks to the power of dense neural input representations that embody global syntactic information. We investigate two conceptually simple local neural models for constituent parsing, which make local decisions to constituent spans and CFG rules, respectively. Consistent with previous findings along the line, our best model gives highly competitive results, achieving the labeled bracketing F1 scores of 92.4% on PTB and 87.3% on CTB 5.1.

==> part/abstract.tex <==
\begin{abstract}
Recent work has shown that state-of-the-art results can be achieved for dependency parsing using a neural network structure inspired by neural machine translation (NMT), which leverages a multi-layer bidirectional LSTM encoder to represent the input sentence, making biaffine attention between the hidden LSTM states to model dependency relations locally. The results are surprising in the sense that no global structured learning is necessary, which has been a major research focus for parsing over the past two decades. This suggests strong representation learning power of LSTM encoders, which implicitly learns output structural dependencies.

We investigate NMT-inspired constituent parsing, using a similar encoder structure without global structural learning to model the task, verifying the effectiveness of LSTM encoders for this task. In particular, we build two simple local models for predicting constituents, one being 0th-order, predicting individual constituents and the other being 1st-order, predicting individual phrase rules. Both models are trained {\it locally}. Experiments show that both models give highly competitive performances compared with the state-of-the-art, again demonstrating strong power of LSTM encoders. Our best models give labeled bracketing F1 score of 92.4\% on PTB and 87.7\% on CTB 5.1, without reranking or ensembling. After reranking, our models further boost the parsing performance. 
\end{abstract}

==> part/abstract1.tex <==
\begin{abstract}
   This paper proposes neural greedy parsers for chart-based constituent parsing, which jointly train an unlabeled constituent tree parser and an encoder-decoder model to generate constituent labels. 
   The unlabeled constituent parser is based on \emph{local} constituent span classification models using simple LSTM features, which requires minimum representation learning, reducing the burden of \emph{global} structure inference. 
   In particular, we presents a \textbf{binary span classification model} to describe the  plausibility of an arbitrary span being a valid constituent span and a  \textbf{biaffine span partition model} to identify the splitting points of constituent spans. 
   Given an unlabeled parsing tree,  an  encoder extracts neural features using lexicalized tree LSTMs  for the decoder to hierarchically generate constituent labels. 
   Experiments show that both binary and biaffine classification models gives better performance compared to the state-of-the-art neural greedy constituent parsers. Our best models give labeled bracketing F1 score of 92.1\% on PTB and 86.8\% on CTB 5.1, without reranking or ensembling. 
\end{abstract}


==> part/analysis.tex <==
\iffalse
\section{Error Analysis}

We analyze the parsing errors of our system using \emph{berkeley-parser-analyser} \cite{Kummerfeld2012EMNLP}.\footnote{https://github.com/jkkummerfeld/berkeley-parser-analyser} 
Table \ref{tab:error} shows the error type distributions of different parsers. CVG is a reranker model based on compositional vector grammars \cite{socher2013parsing}. 
Transition-based Neural Constituent Parser (\emph{TNCP}) \cite{watanabe2015transition}, \emph{RNNG} \cite{kuncoro2017rnng}, Span-based Constituent Parser (\emph{SCP}) \cite{james2016span} are representative transition-based constituent parsers. \emph{Biaffine} denotes our biaffine partition model.  

Overall, \emph{Biaffine} leads to fewer errors compared to \emph{CVG} and \emph{TNCP}. 
Similar to other parsers, the largest errors of \emph{Biaffine} results from PP attachment.  
It is worth noting that \emph{Biaffine}, \emph{RNNG} and \emph{SCP} make different errors.   
Compared with \emph{RNNG}, the main error reductions of \emph{Biaffine} come from  clause attachments (0.46$\rightarrow$0.37), NP attachments (0.29$\rightarrow$0.19), and co-ordinations (0.30$\rightarrow$0.21). While the main difference between \emph{SCP} and \emph{Biaffine} lies in co-ordination errors (0.26 v.s. 0.21) and other errors (0.47 v.s. 0.39) such as ``UNSET add''.  

\begin{table}[!t]
  \centering
  \small
  \setlength{\tabcolsep}{3.5pt}
  \begin{tabular}{|l|c|c|c|c|c|}
  \hline 
  Error Type &  CVG & TNCP & RNNG  & SBCP & Biaffine\\
  \hline
  PP Attach & 0.79 & 0.73 & \bf{0.64} & 0.67 & 0.65  \\
  Clause Attach  & 0.43 & 0.38 &  0.46 & 0.36 & \bf{0.37} \\
  Diff Label & 0.29 & 0.29 & \bf{0.24} & 0.27 & \bf{0.24}\\
  Mod Attach  & 0.27 & 0.27 & 0.23 & 0.22 & \bf{0.21} \\
  NP Attach  & 0.31 & 0.32 & 0.29 & 0.20 & \bf{0.19}\\
  Co-ord  & 0.32 & 0.29 & 0.30& 0.26 & \bf{0.21}\\
  1-Word Span  & 0.31 &  0.30 & \bf{0.24} & 0.27 & \bf{0.24}\\
  Unary & 0.22 & \bf{0.18} &  0.19 & 0.21 & \bf{0.18}\\
  NP Int  & \bf{0.19} & 0.20 & \bf{0.19} & 0.20 & \bf{0.19}\\
  Other  & 0.41 & 0.45 &  0.40 & 0.47 & \bf{0.39}\\
  \hline
  \end{tabular}
  \caption{Distributions of the average number of errors per sentence on the PTB test set by different parsers. We directly cite CVG \protect \cite{socher2013parsing} and TNCP \protect \cite{watanabe2015transition} results from \protect \newcite{watanabe2015transition}, and run the open-source implementations of RNNG \protect \cite{kuncoro2017rnng} and SBCP \protect \cite{james2016span} to obtain their results. \vspace{-1em} } 
  \label{tab:error}
\end{table}
\fi



%\subsection{Converging Speed}
%\subsection{Parsing Speed}
%\subsection{Span length}
%\subsection{Sentence length}

==> part/credit.tex <==
\section{Credits}

This document has been adapted from the instructions for  
COLING-2016 proceedings compiled by Hitoshi Isahara and Masao Utiyama,
which are, in turn, based on
the instructions for
COLING-2014 proceedings compiled by Joachim Wagner, Liadh Kelly
and Lorraine Goeuriot,
which are, in turn, based on the instructions for earlier ACL proceedings,
including 
those for ACL-2014 by Alexander Koller and Yusuke Miyao,
those for ACL-2012 by Maggie Li and Michael
White, those for ACL-2010 by Jing-Shing Chang and Philipp Koehn,
those for ACL-2008 by Johanna D. Moore, Simone Teufel, James Allan,
and Sadaoki Furui, those for ACL-2005 by Hwee Tou Ng and Kemal
Oflazer, those for ACL-2002 by Eugene Charniak and Dekang Lin, and
earlier ACL and EACL formats. Those versions were written by several
people, including John Chen, Henry S. Thompson and Donald
Walker. Additional elements were taken from the formatting
instructions of the {\em International Joint Conference on Artificial
  Intelligence}.


==> part/experiment.tex <==
\section{Experiments}

\subsection{Experimental Settings}

\textbf{Data.} We perform  experiments  for both English and Chinese. 
Following standard conventions, our English data are obtained from the Wall Street Journal (WSJ) of the Penn Treebank (PTB) \cite{marcus1993building}. Sections 02-21, section 22 and section 23 are used for training, development and test sets, respectively. 
Our Chinese data are the version 5.1 of the Penn Chinese Treebank (CTB) \cite{xue2005penn}. The training set consists of articles 001-270 and 440-1151, the development set contains articles 301-325 and the test set includes articles 271-300. We use automatically reassigned POS tags in the same way as \newcite{james2016span} for English and \newcite{dyer2016rnng} for Chinese. 

We use ZPar \cite{zhang2011syntactic}\footnote{https://github.com/SUTDNLP/ZPar} to binarize both English and Chinese data using  head rules of \newcite{collins2003head}.  The head directions of the binarization results are ignored during training. The types of English and Chinese constituent span labels after binarization are 52 and 56, respectively. We limit the maximum number of greedy decoding steps for generating consecutive constituent labels to be 4 for both English and Chinese, as suggested by the treebanks.  

\textbf{Evaluation.} We evaluate parsing performance in terms of both unlabeled bracketing metrics and labeled bracketing metrics including unlabeled F1 (UF), labeled precision (LP), labeled recall (LR) and labeled bracketing F1 (LF) after debinarization using EVALB\footnote{http://nlp.cs.nyu.edu/evalb}.  

\textbf{Unknown words.} Unknown word processing is usually discussed in neural parsing models \cite{dyer2016rnng,james2016span,KiperwasserG16a}. 
For English, we combine the ways of \newcite{dyer2016rnng} and \newcite{james2016span} to handle unknown words. We first map all words (not just singleton words) in the training corpus into unknown word classes using the same rule as \newcite{dyer2016rnng}.  During each training epoch, every word $w$ in the training corpus is stochastically mapped into its corresponding unknown word class $unk_w$ with probability $P( w \rightarrow unk_w) = \frac{ \gamma } {  \gamma + \#w }$, where $\#w$ is the frequency count and $\gamma$ is a control parameter. 
Intuitively, the more times a word appears, the less opportunity it will be mapped into its unknown word type. There are 54  unknown word types for English.  Following \newcite{james2016span}, $\gamma=0.8375$.  
For Chinese, we simply use one unknown word type to dynamically replace singletons words with a probability of 0.5.  

\begin{table}[!t]
    \centering
    \small
    \setlength{\tabcolsep}{3.5pt}
  \begin{tabular}{l|c|l|c}
    \hline
    \bf hyper-parameter & \bf value & \bf hyper-parameter & \bf value\\
    \hline
    Word embeddings & English: 100 Chinese: 80 &
    Word LSTM layers & 2  \\
    Word LSTM hidden units & 200 &
    Character embeddings & 20 \\
    Character LSTM layers & 1 &
    Character LSTM hidden units & 25 \\
    Tree-LSTM hidden units & 200 &
    POS tag embeddings & 32 \\
    Constituent label embeddings & 32 & 
    Label LSTM layers & 1 \\
    Label LSTM hidden units & 200 & 
    Last output layer hidden units & 128 \\
    Maximum training epochs & 50 &
    Dropout & English: 0.5, Chinese 0.3 \\
    Trainer & SGD &
    Initial learning rate & 0.1 \\
    Per-epoch decay & 0.05 &
    $\phi$ & $\textsc{ELU}$ \cite{elu2015} \\
    \hline
   \end{tabular}
   \caption{Hyper-parameters for training. \vspace{-1.5em}}
  \label{tab:hyper}
\end{table}

 \textbf{Hyper-parameters.}  Table \ref{tab:hyper} shows all hyper-parameters. These values are tuned using the corresponding development sets. We optimize our models with  stochastic gradient descent (SGD).  The initial learning rate is 0.1.  We initialize our model with pretrained word embeddings both for English and Chinese. The pretrained word embeddings are the same as those used in \newcite{dyer2016rnng}. Other parameters are initialized according to the default settings of DyNet \cite{neubig2017dynet}. We apply dropout \cite{srivastava2014dropout} to the inputs of every LSTM layer, including the word LSTM layers, the character LSTM layers,  the tree-structured LSTM layers and the constituent label LSTM layers. For Chinese, we find that 0.3 is a good choice for dropout probability. The number of training epochs is decided by the evaluation performances on development set. In particular, we perform evaluations on development set for every 10,000 examples.  The training procedure stops when the results of next 20 evaluations do not become better than the previous best record.

\subsection{Development Results}
\textbf{Span Representation.} We mentioned two span representation methods, namely the simple concatenating representation $\mathbf{v}[i,j]$ in Eq \ref{eq:v} and the  combining of three difference vectors $\mathbf{sr}[i,j]$ in Eq \ref{eq:spanrep}. We investigate appropriate representations for different models on the English dev  dataset. We use two representative models, i.e, the BinaryClas model  and the biaffine partition BiaffinePartition rule model, as studying objects. Table \ref{tab:repcompare} shows the affects of  different span representation methods for these two models. We verify that $\mathbf{v}[i,j]$ is better for the BinaryClas model and $\mathbf{sr}[i,j]$ is better for the BiaffinePartition model. When using $\mathbf{sr}[i,j]$ for the BinaryClas model, the performance drops greatly ($92.17\rightarrow 91.80$). Similar observations can be found when replacing $\mathbf{sr}[i,j]$ with $\mathbf{v}[i,j]$ for the  BiaffinePartion model. Therefore, we use $\mathbf{v}[i,j]$ for the span models and $\mathbf{sr}[i,j]$ for the rule  models in latter experiments.  

\textbf{Main dev results.} Table \ref{tab:maindev} shows the main results on English dev set and Chinese dev set. For English, the BinaryClas model  acheives 92.17 LF score. The classifier MultiClas is much better than the BinaryClas model due to the awareness of label information. Simliar phenomenon can be observed on the Chinese dataset.  For English,  we also try linear scoring methods. The LinearPartition model obtains 92.03 LF score, which is much worse than the BiaffinePartition model.  
In general, the performances of the BiaffinePartition model, and the MultiSpanClas model are quite close both for English and Chinese. 
\begin{table*}[!t]
\small
\setlength{\tabcolsep}{3.0pt}
\begin{minipage}{.5\linewidth}
\centering
\begin{tabular}{l|c|c|c|c|c|c}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{English} & \multicolumn{3}{c}{Chinese} \\
\cline{2-7}
      & LP & LR & LF & LP & LR & LF\\
     \hline
     BinaryClas & 92.16 &	92.19 &	92.17 & 91.31 & 90.48 & 90.89\\
     MultiClas & 92.47	& \bf 92.41	& \bf 92.44 & \bf 91.69	& 90.91	& \bf 91.30\\
     \hline 
     Biaffine & \bf 92.49 &	92.23 & 92.36& 91.31 &	\bf 91.28	& 91.29\\
\hline 
\end{tabular}
\caption{Main development results.}
\label{tab:maindev}
\end{minipage}
\begin{minipage}{.5\linewidth}  
\centering
\begin{tabular}{l|l|c|c|c}
    \hline 
        Model & SpanVec & LP & LR & LF \\
        \hline 
        \multirow{ 2}{*}{BinaryClas} & $\mathbf{v}[i,j]$ & \bf 92.16 & \bf 92.19 & \bf 92.17 \\
          & $\mathbf{sr}[i,j]$ & 91.90	& 91.70 & 91.80 \\
        \hline 
       \multirow{ 2}{*}{BiaffinePartition}  & $\mathbf{v}[i,j]$ & 91.79 &	91.67 &	91.73 \\
         & $\mathbf{sr}[i,j]$ & \bf 92.49 &	\bf 92.23 &	\bf 92.36 \\
        \hline
    \end{tabular} 
  \caption{Span representation methods.}
    \label{tab:repcompare} 
\end{minipage}  
\end{table*}
\subsection{Main Results}

\textbf{English.} Table \ref{tab:expeng} summarizes the performances of various constituent parsers on PTB test set.  Our binary classification model and biaffine partition model achieves similar labeled F1 scores, which are both better than the state-of-the-art neural greedy transition-based parsing models \cite{james2016span,kuncoro2017rnng}. 
In addition, our neural local parsing models outperform the state-of-the-art neural CKY parsing models \cite{durrett2015crf} ($91.1\rightarrow92.1$), which integrates neural features and sparse features into a CRF-based parser. 


\begin{table}[!t]
  \centering
  \small
  \setlength{\tabcolsep}{3.5pt}
  \begin{tabular}{l|l|l|l|l|l|l|l}
    \hline
    Parser       & LR & LP &  LF & Parser       & LR & LP &  LF\\
    \hline
    \newcite{charniak2000maximum}&  89.5 & 89.9 & 89.5 &
    \newcite{collins2003head} & 88.1 & 88.3 & 88.2 \\
    \newcite{sagae2006combine} & 87.8 & 88.1 & 87.9 &
    \newcite{petrov2007unlex} & 90.1 & 90.2 & 90.1 \\
    \newcite{carreras2008tag} & 90.7 & 91.4 & 91.1 &
    \newcite{zhu2013acl} & 90.2 & 90.7 & 90.4 \\
    \newcite{vinyals2015grammar}  & & & 88.3 &
    \newcite{watanabe2015transition} & & & 90.7\\
    \newcite{fernandezgonzalez-martins:2015:ACL-IJCNLP} & 89.9 & 90.4 & 90.2 &
    \newcite{james2016span}& 90.5 & 92.1 & 91.3 \\ 
    \newcite{liu2016lookahead} & 91.3 & 92.1 & 91.7 &
    \newcite{kuncoro2017rnng}  & & & 91.2   \\
    \newcite{sternandreasklein:2017:Long} top-down & 90.4 & 93.2 & 91.8 &
    \newcite{mcclosky2006rerank} (S) & 92.1 & 92.5 & 92.3 \\
    \newcite{zhu2013acl} (S) & 91.1 & 91.5 & 91.3 & 
    \newcite{durrett2015crf} (S) & & & 91.1 \\
    \newcite{choe2016parsinglm} (S,R,E) & & & 93.8 &
    \newcite{vinyals2015grammar} (S, E) & & & 92.8 \\
    \newcite{charniak2005rerank} (S, R) & 91.2 & 91.8 & 91.5 &
    \newcite{huang2008forest} (R) & & & 91.7 \\
    \newcite{huang2009selftraining} (ST) & 91.1 & 91.6 & 91.3 &
    \newcite{huang2010product} (ST) & 92.7 & 92.2 & 92.5 \\
    \newcite{shindo2012refined} (E) & & & 92.4 & 
    \newcite{socher2013parsing} (R) & & & 90.4 \\
    \newcite{vinyals2015grammar} (E) & & & 90.5 &
    \newcite{choe2016parsinglm} (R) & &  & 92.6 \\
    \newcite{dyer2016rnng} (R) & & & 93.3   & 
    \newcite{kuncoro2017rnng} (R) & & & 93.6 \\ 
    \newcite{liu2017inorder} (R) & & & 94.2 & 
    \newcite{fried-stern-klein:2017:Short} (ES) & & & \bf 94.7 \\
    \hline
    \multicolumn{4}{c|}{\multirow{3}{*}{Our work}} &  BinarySpanClas & 91.9 & 92.2 &	92.1 \\ 
    \multicolumn{4}{c|}{} & MultiSpanClas & 92.2 &	92.5 & 92.4 \\
    \multicolumn{4}{c|}{} & BiaffinePartition & 92.0 & 92.6  &	92.3 \\
    \hline
  \end{tabular}
  \caption{Results on the PTB test set.  \emph{S} denotes parsers using auto parsed trees. \emph{E}, \emph{R} and \emph{ST} denote ensembling, reranking and self-training systems, respectively.  \vspace{-1.5em}}
  \label{tab:expeng}
\end{table}


\textbf{Chinese.} Table \ref{tab:expchn} shows the parsing performance on CTB 5.1 test set. Both our binary classification model and biaffine partition model outperform the state-of-the-art neural greedy model \cite{dyer2016rnng}, improving the labeled F1 score by 2.4 at most.  The biaffine partition model is better than the binary classification model on this test set (86.35 v.s. 86.82). In addition, the biaffine partition model achieves performance close to the generative reranking systems using recurrent neural network grammars \cite{dyer2016rnng} and methods that do joint POS tagging and parsing \cite{wang2014joint,wang2015feature}.


\begin{table}[!t]
  \centering
  \small
  \setlength{\tabcolsep}{3.5pt}
  \begin{tabular}{l|l|l|l|l|l|l|l}
    \hline
    Parser   &    LR & LP &  LF & Parser   &    LR & LP &  LF \\
    \hline
    \newcite{charniak2000maximum}& 79.6 & 82.1 & 80.8 &
    \newcite{bikel2004parameter} & 79.3 &  82.0 & 80.6 \\
    \newcite{petrov2007unlex} & 81.9 & 84.8 & 83.3 &
    \newcite{zhang2009tran} & 78.6 & 78.0 & 78.3\\
    \newcite{huang2009selftraining}& & & 84.2 &
    \newcite{zhu2013acl} & & & 83.2 \\
    \newcite{wang2015feature} & & & 83.2 &
    \newcite{watanabe2015transition} & & & 84.3 \\
    $\ddagger$\newcite{dyer2016rnng} & & & 84.6   &
    \newcite{liu2016lookahead} & 85.2 & 85.9  & 85.5 \\
    \newcite{liu2017inorder} & & & 86.1 &
    \newcite{charniak2005rerank} (R) & 80.8 & 83.8 &  82.3 \\
    \newcite{zhu2013acl} (S) & 84.4 & 86.8 & 85.6 &
    \newcite{wang2014joint} (S) & & & 86.3 \\
    \newcite{wang2015feature} (S) & & & 86.6 &
    \newcite{huang2009selftraining} (ST) & & & 85.2 \\
    \newcite{dyer2016rnng} (R) & & & 86.9   &
    \newcite{liu2017inorder} (R) & & & 88.0 \\
    \hline
    \multicolumn{4}{c|}{\multirow{3}{*}{Our work}} & {BinaryClas}   & 85.9 & 87.1 & 86.5 \\
    \multicolumn{4}{c|}{} & {MultiClas} & 86.6 & 88.0		& 87.3 \\
    \multicolumn{4}{c|}{} & {BiaffinePartition}&	87.1 & 87.5  & 87.3 \\
  \end{tabular}
  \caption{Results on the Chinese Treebank 5.1 test set.  \emph{S} denotes parsers using auto parsed trees. \emph{R} and \emph{ST} denote reranking and self-training systems, respectively. \vspace{-1em} }
  \label{tab:expchn}
\end{table}


==> part/intro.tex <==
\section{Introduction}

Constituent parsing has traditionally been tackled as a structured-learning task, where the training objective is to globally optimize a set of inter-dependent decisions for disambiguating overall output structures. 
Typical methods can be classified into graph-based models, which directly score phrase-structure rules in output constituent trees, and transition-based models, which map the output-building process as a state-transition process, using a sequence of transition actions to construct outputs incrementally. Output constituent trees are measured indirectly by scoring their corresponding sequences of transition actions.

Neural network models have been proposed for both graph-based \cite{durrett2015crf} and transition-based \cite{watanabe2015transition,wang2014joint,cross2016bilstm} constituent parsing, giving results that are competitive to the best statistical counterparts. Most work in this line can be viewed as using a neural network to substitute \cite{watanabe2015transition,dyer2016rnng} or complement \cite{durrett2015crf,liu2016lookahead} a statistical model for structured prediction, exploiting the strength of neural representation learning for extracting dense feature representations. 

There has been work using deep neural networks to learn a global representation of the whole input sentence, before making parsing decisions. Such methods have taken inspiration from neural machine translation, for which the dominant approach uses an encoder-decoder structure, learning a dense vector representation of the input, before generating the output \cite{cho2014properties}. The same encoder-decoder architecture has been used for constituent parsing \cite{vinyals2015grammar}, with the input being taken as the ``source language'' and the ``target language'' being a linearized form of constituent trees via bracketed notation. While \newcite{vinyals2015grammar}  observe reasonable performance on standard benchmarks, a limitation has been recognized for the model is not explicitly modelling salient structures in the output \cite{dyer2016rnng}. 

The potentials of the encoder structure has been demonstrated by a more promising strand of methods in dependency parsing \cite{KiperwasserG16a,Dozat2016biaffine}, which replaces the decoder structure with explicit modelling of bi-word relations based on encoder hidden states of each words in a given sentence. For decoding, a simple spanning tree algorithm that integrates local arc scores can be applied, without inter-arc structure patterns being considered. Surprisingly, without considering global structural relations during learning, such methods give results that are highly comparable to both graph-based and transition-based models that employ structured learning, with the method of \newcite{Dozat2016biaffine} giving the best reported results among direct dependency parsing models. 

The observation demonstrates the power of multi-layer bidirectional LSTMs (BiLSTM) \cite{hochreiter1997long,graves2013hybrid} in capturing non-local \emph{output} dependency information over \emph{input} sentences, since hidden states for each word can contain sufficient information to allow local arc models to contain global structural information, without suffering label bias. Intuitively, such strength can benefit not only dependency parsing, but constituent parsing also, which takes a different form of linguistic structures. We verify this hypothesis by building two NMT-inspired constituent parsing models without structured learning, relying solely on a multi-layer BiLSTM encoder to represent input sentences. For decoding, our models make local decisions on the existence of unlabeled constituent spans first, before labeling each consistent and making unary rule decisions.

In particular, for unlabeled constituent recognition, our first model makes 0/1 decisions on each constituent span on a CKY chart locally according to the hidden LSTM states of the beginning and ending words. Our second model considers span partition top-down. Starting from the sentence-level span, it makes local disambiguations on the partition point  of a binary phrase-structure rule recursively. Results on the standard WSJ benchmark show that both forms of decoding give comparable accuracies. Our models outperform the best graph-based and transition-based constituent parser models, giving the best results without using ensembling or semi-supervised learning. This demonstrates the usefulness of NMT-style LSTM encoders  for learning constituent syntax information.
 
 We release our code at \url{http://anonymized}.

==> part/intro1.tex <==
\section{Introduction}
Non-local features have been shown crucial for statistical parsing \cite{huang:2008:ACLMain,zhangnivre2011transition}. 
For dependency parsing, High-order dynamic programs \cite{koocollins:2010:ACL}, integer linear programming \cite{martins:2010:EMNLP} and dual decomposition \cite{koo:2010:EMNLP} techniques have been exploited by graph-based parser to integrate non-local features. Transition-based parsers \cite{Nivre03anefficient,Nivre:2008:CL,zhangnivre2011transition,bohnet:2010:coling,huangfayongguo:2012:NAACL} are also known for leveraging non-local features for achieving high accuracies. For most state-of-the-art statistical parsers, a global training objective over the entire parse tree has been defined to avoid label bias \cite{lafferty2001conditional}.

For neural parsing, on the other hand, locally-trained models have been shown to give highly competitive accuracies \cite{chen2014dep,dyer:2015:stack,james2016span,sternandreasklein:2017:Long}, as compared to those that employ a global sentence-level loss \cite{watanabe2015transition,zhou:2015:sentloss,andor:2016:global,durrett2015crf}. In addition, highly local features have been used in recent state-of-the-art models \newcite{sternandreasklein:2017:Long,Dozat2016biaffine}. In particular, \newcite{Dozat2016biaffine} show that a locally trained arc-factored model can give the best reported accuracies on dependency parsing. The surprising result has been largely attributed to the representation power of LSTM encoders \cite{KiperwasserG16a}.

An interesting research questions is to what extent the encoding power can be leveraged for constituent parsing. We investigate the strength of the encoder structure by building a model that is local to unlabelled constituent spans \cite{abney1991parsing}.   One other rudimentary structure is CFG-rules, which has been explored by early PCFG models \cite{collins2003head,klein2003unlex}. For comparison with our span level model, we build a second  model local to unlabelled CFG rules, leveraging bi-affine modelling \cite{Dozat2016biaffine} for predicting rule-level accuracies. Constituent labels are assigned on unlabeled trees by using a tree-LSTM to encode the syntactic structure, and a LSTM decoder for yielding label sequences on each node, which can include unary rules. 

Experiments show that our models  give highly competitive performances compared with the state-of-the-art,  demonstrating strong power of local  models. Our best models give labeled bracketing F1 score of 92.4\% on PTB and 87.3\% on CTB 5.1, without reranking or ensembling.





==> part/model.tex <==
\section{Model}
\begin{figure*}[!t]
\begin{subfigure}[b]{0.5\textwidth}
   \includegraphics[width=\textwidth]{pics/spanclas2.pdf}
   \caption{BiLSTM based constituent span classifier.   }
   \label{fig:spanclas}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\small
\begin{tikzpicture}
\Tree 
[.$[0,4]$ 
    [.$[0,2]$ 
        [.$[0,0]$ DT\\{The$_0$} ] 
        [.$[1,2]$ 
            [.[1,1] NN\\{stock$_1$} ] 
            [.[2,2] NN\\{price$_2$} ] 
        ] 
    ] 
    [.$[3,4]$ 
        [.[3,3] VBZ\\{keeps$_3$} ]
        [.[4,4] VBG\\{falling$_4$} ]  
    ] 
]
\end{tikzpicture}
\caption{Unlabeled binarized parse tree.}
\label{fig:binarized}
\end{subfigure}

\begin{subfigure}[b]{0.5\textwidth}
\centering
\small
\begin{tikzpicture}
\Tree 
[.[0,4]:S$\rightarrow \phi$
    [.[0,2]:NP$\rightarrow \phi$ 
        [.[0,0]:$\phi$ 
            DT\\{The$_0$} 
        ] 
        [.[1,2]:NP*$\rightarrow \phi$ 
            [.[1,1]:$\phi$ NN\\{stock$_1$} ] 
            [.[2,2]:$\phi$ NN\\{price$_2$} ] 
        ] 
    ] 
    [.[3,4]:VP$\rightarrow \phi$ 
        [.[3,3]:$\phi$ VBZ\\{keeps$_3$} ] 
        [.[4,4]:VP$\rightarrow$S$\rightarrow \phi$ VBG\\{falling$_4$} ]   
    ] 
]
\end{tikzpicture}
\caption{Label generator. \textbf{NP*} is an intermediate constituent label. $\phi$ is an ending marker.}
\label{fig:binlabeltree}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \small
\begin{tikzpicture}
\Tree 
[.S$[0,4]$ 
    [.NP$[0,2]$ DT\\{The$_0$} NN\\{stock$_1$} NN\\{price$_2$} ] 
    [.VP$[3,4]$ VBZ\\{keeps$_3$} 
        [.S$[4,4]$ 
            [.VP$[4,4]$ VBG\\{falling$_4$} ] 
        ] 
    ] 
]
\end{tikzpicture}
\caption{Final example parse tree.}
\label{fig:fulltree}
\end{subfigure}
\caption{An overview workflow of our chart-based neural greedy constituent parser for processing the sentence ``The stock price keeps falling''. We annotate every non-terminal span with its covered span range. Figure \ref{fig:spanclas} shows constituent span classifiers making 0/1 decisions for all possible spans. Based on the local classification probabilities, we obtain an unlabeled binarized parse tree (Figure \ref{fig:binarized}) using binary CKY parsing algorithms. We then hierarchically generate labels for each span (Figure \ref{fig:binlabeltree}) using encoder-decoder models. Figure \ref{fig:fulltree} shows the final output parse tree after debinarization. }
\label{fig:all}
\end{figure*}


Our models consist of an unlabeled binarized tree parser and a label generator. 
Figure \ref{fig:all} shows a running example of our parsing model.  
The unlabeled parser (Figure \ref{fig:spanclas}, \ref{fig:binarized}) learns an unlabeled parse tree using simple BiLSTM encoders.  The label generator (Figure \ref{fig:binlabeltree}, \ref{fig:fulltree})  predicts constituent labels for each span in the unlabeled tree using encoder-decoder models. 

The unlabeled parser employs classification models to describe the probability $p([i, j] \rightarrow [i, k] [k+1, j])$ of the span production rule that the span $[i, j]$ is composed by two children spans $[i, k]$ and $[k+1, j]$ where $i\leq k < j$.  
We then use the CKY algorithm to derive unlabeled binarized parse trees based on span production probabilities,  

In particular, we design two different classification models for unlabeled parsing: the \textbf{binary classification model} (Section \ref{sec:binary}) and the \textbf{biaffine partition model} (Section \ref{sec:biaffine}). 
The binary classification model identifies the probability of an arbitrary span being a constituent span. 
For example, the span [1,2] in Figure \ref{fig:spanclas} belongs to the correct parse tree (Figure \ref{fig:fulltree}). Ideally, our model assigns a high probability to this span.  
In contrast, the span [0,3] is not a valid constituent span and our model labels it with 0. 
Different from the binary classification model,  the biaffine partition model directly considers the probability of the splitting point $k$ ($i\leq k \leq j$) for a span $[i,j]$ using the biaffine scoring network \cite{Dozat2016biaffine}.  For example, in Figure \ref{fig:spanclas}, $k=0$ is a better partition point for span $[0, 2]$ than $k=1$. Therefore, the biaffine model assigns high probability to the rule $[0, 2] \rightarrow [0, 0] [1, 2]$ instead of $[0, 2] \rightarrow [0, 1] [2, 2]$.  

The label generator adopts a encoder-decoder \cite{cho2014properties,sutskever2014sequence} framework to encode a binarized unlabeled tree and to decode constituent labels for every span. 
The encoder is a  binary tree-LSTM encoder \cite{tai15treelstm,zhu15treelstm} which composes the representation vector for tree nodes in a bottom-up style. 
Base on the representation vector of a constituent span, the decoder generates chains of constituent labels. For example, the decoder outputs ``VP $\rightarrow$S$ \rightarrow \phi$'' for the span [4, 4]  and ``NP$\rightarrow \phi$'' for the span [0,2] in Figure \ref{fig:binlabeltree} where $\phi$ is a stopping symbol. 


\subsection{Binary Span Classification Model}
\label{sec:binary}

 Given an unlabeled binarized tree $T_{ub}$ for the sentence $S$, $S= w_0, w_1 \dots w_{n-1}$,  the binary classification model trains a neural network model $P(Y_{[i,j]}|S, \Theta)$ to distinguish  constituent spans from  non-constituent spans, where $0 \leq i \leq n-2$, $ 1 \leq j < n$, $i < j$, $Y_{[i, j]} =1 $ indicate the span [i, j] is a constituent span ($[i, j] \in T_{ub}$), and  $Y_{[i, j]} =0 $ for otherwise, $\Theta$ are model parameters.  We do not model spans with length 1 since the span [i, i] always belongs to $T_{ub}$. 


\textbf{Network Structure.} Figure \ref{fig:binclas} shows the neural network structures for the binary classification model. In the bottom, a bidirectional LSTM layer encodes the input sentence to extract non-local features. In particular, we append a starting symbol $<$s$>$ and an ending symbol $<$/s$>$ to the left-to-right LSTM and the right-to-left LSTM, respectively.   We denote the output hidden vectors of the left-to-right LSTM and the right-to-left LSTM  for $w_0, w_1, \dots, w_{n-1}$ 
are $\mathbf{f}_1, \mathbf{f}_2, \dots, \mathbf{f}_n$ and $\mathbf{r}_0, \mathbf{r}_1, \dots, \mathbf{r}_{n-1}$, respectively.  
We obtain the representation vector $\mathbf{v}[i, j]$ of the span $[i, j]$ by simply concatenating the bidirectional output vectors at the input word $i$ and the input word $j$,
\begin{equation}
\mathbf{v}[i,j]=[\mathbf{f}_{i+1};\mathbf{r}_{i}; \mathbf{f}_{j+1}; \mathbf{r}_{j}].
\label{eq:v}
\end{equation}
We then pass $v[i, j]$ through a nonlinear transformation and get the probability distribution 
$P(Y_{[i,j]})$ by
\begin{equation*}
    \begin{split}
        \mathbf{o}[i,j] &= \tanh (\mathbf{W_o} \mathbf{v}[i,j] + \mathbf{b_o}) \\
        \mathbf{u}[i,j] &= \mathbf{W_u} \mathbf{o}[i,j] + \mathbf{b_u} \\
        P(Y_{[i,j]}) &= \text{softmax}(\mathbf{u}[i,j]), \\
    \end{split}
\end{equation*}
where $\mathbf{W}_o, \mathbf{b}_o, \mathbf{W}_h$ and $\mathbf{b}_h$ are model parameters. 

\textbf{Input Representation.} For the parsing tasks, the input sentence usually contains words and part-of-speech (POS) tags, we combine them together to obtain the input representation vectors. Figure \ref{fig:input} shows the neural network architecture.  Given a word $w$, its corresponding characters $c_0,\dots, c_{|w|-1}$ and POS tag $t$, firstly, we get the word embedding $\mathbf{E}_{word}^w$, character embeddings $\mathbf{E}_{char}^{c_0},\dots, \mathbf{E}_{char}^{c_{|w|-1}}$, and POS tag embedding $\mathbf{E}_{pos}^t$ using lookup operations. Then we use a bidirectional LSTM to extract character-level features. Suppose the output vectors of the last step of the left-to-right and right-to-left LSTMs are $\mathbf{h}_{char}^f$ and $\mathbf{h}_{char}^r$, respectively.  The final input vector $\mathbf{x}_{input}$ is given by 
\begin{equation}
    \begin{split}
        &\mathbf{x}_{char} = \tanh (\mathbf{W}_{char}^f \mathbf{h}_c^f +  \mathbf{W}_{char}^r \mathbf{h}_c^r + \mathbf{b}_{char} ) \\
        &\mathbf{x}_{input} = [ \mathbf{E}_{word}^w + \mathbf{x}_{char};  \mathbf{E}_{pos}^t],\\
    \end{split}
    \label{eq:xinput}
\end{equation}
where $\mathbf{W}_{char}^f$, $\mathbf{W}_{char}^r$ and $\mathbf{b}_{char}$ are model parameters. 
\newcite{wang2015char} demonstrated that the input representation vector $\mathbf{E}_{word}^w + \mathbf{x}_{char}$ obtained the-state-of-the-art POS tagging accuracy.  Inspired by their experiments, we design this network to combine words, characters and POS tags as input representations for constituent parsing.

\begin{figure}[!t]
   \includegraphics[width=0.5\textwidth]{pics/conparsingrep.pdf}
   \caption{Neural network architectures for composing words, characters and POS tags.}
   \label{fig:input}
\end{figure}

\textbf{Training objective.} The training objective is to maximize the probabilities of $P(Y_{[i,j]=1}|S, \Theta)$ for spans $[i,j] \in T_{ub}$ and minimize the probabilities of $P(Y_{[i,j]=1}|S, \Theta)$ for spans $[i,j] \notin T_{ub}$ at the same time. 
Formally, the training loss for binary span classification $L_{\text{span}}$ is given by
\begin{equation}
\begin{split}
    L_{\text{binary}} &= -\sum_{[i,j] \in T_{ub}}{ \log p(Y_{[i,j]} = 1 | S, \Theta)}   \\
    &-\sum_{[i,j] \notin T_{ub}}{ \log p(Y_{[i,j]} = 0 |S, \Theta)}, \\
    & (0 \leq i \leq n-2, 1 \leq j < n, i < j)
\end{split}
\label{eq:binloss}
\end{equation}
For a sentence with length $n$, there are $\frac{ n (n -1) } {2}$ terms in total in Equation \ref{eq:binloss}. 


\begin{figure*}[!t]
\begin{subfigure}[b]{0.48\textwidth}
   \includegraphics[width=\textwidth]{pics/binaryclas.pdf}
   \caption{Binary span classification model.   }
   \label{fig:binclas}
\end{subfigure}
\begin{subfigure}[b]{0.48\textwidth}
   \includegraphics[width=\textwidth]{pics/biaffinescore.pdf}
   \caption{Biaffine span partition model.   }
   \label{fig:biaffine}
\end{subfigure}
\caption{Two different models for constituent span classification using BiLSTM encoders.}
\label{fig:model}
\end{figure*}



\textbf{Neural CKY algorithm.} The unlabeled production probability for the rule $r:[i, j]\rightarrow[i, k][k+1, j]$  given by the binary classification model is,  
\begin{equation*}
\begin{split}
P(r | S, \Theta)  = &P( Y_{[i, k]} = 1 |S, \Theta ) * \\
&P( Y_{[k+1, j]} = 1 |S, \Theta) \\
\end{split}
\end{equation*}

During decoding, we find the optimal parse tree $T_{ub}^{*}$ by 
\begin{equation}
    \begin{split}
        T_{ub}^{*} &= \argmax_{T_{ub}} P(T_{ub} | S, \Theta) \\
                   &= \argmax_{T_{ub}} \prod_{r \in T_{ub} } P( r |  S, \Theta) \\
                   &= \argmax_{T_{ub} } \prod_{[i, j] \in T_{ub} } P( Y_{[i,j]}=1 |  S, \Theta)\\
    \end{split}
    \label{eq:decode}
\end{equation}

According to Equation \ref{eq:decode}, we use the CKY algorithm to find $T_{ub}^{*}$.
Algorithm 1 shows the decoding procedure. Lines 1-5 initialize the chart cell score $C[i, j]$ with the probability distribution obtained from the neural network classification model. Lines 6-16 show the standard dynamic programming algorithm.  Lines 10 - 14 find a optimal subtree for the span $[i, j]$. Line 16  updates the chart cell score so that $C[i,j]$ stands for the probability of the optimal subtree spanning $[i, j]$.  During decoding, we maintain backtracing pointer $B[i,j]$ which records the optimal splitting point of cell $[i, j]$ to infer the final optimal tree. 

\begin{algorithm}[!t]
 \KwData{Input sentence $S$, model parameters $\Theta$, sentence length $n$, cell scores $C$, backtracing pointers $B$. }
 \KwResult{an unlabeled parsing tree $t$. }
 \For{\texttt{i=0; i<n; i++}}{
    C[i, i] = 0 \;
 }
 \For{\texttt{i=0; i< n; i++}}{
    \For{\texttt{j = i+1; j < n; j++}}{
        C[i, j] = $\log p(Y_{[i,j]}=1 \vert S, \Theta)$ \;
    }
 }
 \For{\texttt{l=2; l <=n; l++}}{
     \For{\texttt{i=0; i+l<= n; i++}}{
        j = i + l - 1 \;
        maxk = i, maxp = $-\infty$\;
        \For{\texttt{k = i; k < j; k++}}{
            cp = C[i, k] + C[k+1, j] \;
            \If{\texttt{maxp < cp} }{
                maxk = k \;
                maxp = cp \;
            }
        }
        B[i, j] = maxk \;
        C[i, j] += maxp \;
      }
  }
  Get tree $t$ from B using backtrace\;
 \caption{Neural CKY parsing.}
  \label{alg:bincky}
\end{algorithm}

Note that this CYK algorithm is different from the standard CKY algorithm mainly in that there is no phrase rule probabilities $p([i, j] \rightarrow [i, k][k+1, j])$ being involved. Hence our model can be regarded as a 0-order constituent tree model, which is the most {\it local}. All structural relations in a constituent tree must be implicitly captured by the BiLSTM encoder over the sentence alone. 

\subsection{Biaffine Span Partition Model}
\label{sec:biaffine}

Inspired by the success of deep biaffine models for dependency parsing \cite{Dozat2016biaffine,ma2017neural}, we propose a biaffine span partition model for unlabeled parsing. 
Instead of doing binary classification, the biaffine model aims at variable-sized classification.  The biaffine model directly calculates the probabilities of all possible splitting points $k$ ($ i\leq k < j)$ for the span $[i, j]$. 
Since the possible splitting points for spans are varied with the length of span, we hypothesize the biaffine model also works for constituent parsing. 

Figure \ref{fig:biaffine} shows the network architecture for the biaffine model by taking the partition point $k=1$ for the span $[1, 3]$ as an example. 
The BiLSTM encoder layer in the bottom is the same as that in the previous binary classification model. We obtain the span representation vectors using difference vectors \cite{wang2016graph,james2016span}. Formally, the span representation vector $\mathbf{sr}[i, j]$ is given by, 
\begin{equation*}
    \begin{split}
        &\mathbf{s}[i, j]=[\mathbf{f}_{j+1} - \mathbf{f}_{i}; \mathbf{r}_{i} - \mathbf{r}_{j+1}] \\
        &\mathbf{sr}[i, j]=[ \mathbf{s}[0, i-1]; \mathbf{s}[i, j]; \mathbf{s}[j+1, n-1]]. \\
    \end{split}
    \label{eq:spanrep}
\end{equation*}
We first combine the difference vectors $(\mathbf{f}_{j+1} - \mathbf{f}_{i})$ and $(\mathbf{r}_{i} - \mathbf{r}_{j+1})$ to get a simple span representation vector $\mathbf{s}[i, j]$.  
In order to take more contextual information such as $f_p$ where $p>j+1$ and $r_q$ where $q<i$, we concatenate $\mathbf{s}[0, i-1]$,  $\mathbf{s}[i, j]$, and $\mathbf{s}[j+1, n-1]$ together to produce the final span representation vector $\mathbf{sr}[i, j]$.  We then transform $\mathbf{sr}[i,j]$ to get a output vector $\mathbf{r}[i,j]$ using a rectifier activation function to exploit the representation power of nonlinear span features,
\begin{equation}
         \mathbf{r}[i,j] = \text{rectify} (\mathbf{W}_r^{M} \mathbf{sr}[i,j] + \mathbf{b}_r^{M}), 
\end{equation}
where $\mathbf{W}_r^{M}$ and $\mathbf{b}_r^{M}$ and model parameters, and $M$ is a parameter set index. We use separate parameters for the rectify layer. $M=P$, $M=L$ and $M=R$ are for the parent span $[i, j]$, the left child span $[i,k]$ and the right child span $[k+1, j]$, respectively.  

We then obtain the score ${lps}_k$ between the parent span $[i,j]$ and the left child span $[i, k]$ using a biaffine scorer
\begin{equation}
\begin{split}
         {lps}_k = &\mathbf{r}[i,j]^{T} \mathbf{W}_{pl} \mathbf{r}[i,k] + \\
                          &(\mathbf{r}[i,j] \oplus \mathbf{r}[i,k]) ^{T} \mathbf{b}_{pl}, \\
\end{split}
\end{equation}
where $\mathbf{W}_{pl}$ and $\mathbf{b}_{pl}$ are model parameters. 
Similarly, we calculate the score ${rps}_k$ between the parent span $[i,j]$ and the right child span $[k+1, j]$ using $\mathbf{W}_{pr}$ and $\mathbf{b}_{pr}$ as parameters.  The overall partition score ${ps}_k$ is therefore given by 
\[
{ps}_k  = {lps}_k + {rps}_k.
\]
In this way, the unlabeled production probability for the rule $r:[i, j]\rightarrow[i, k][k+1, j]$ is, 
\begin{equation*}
     p([i, j] \rightarrow [i, k] [k+1, j]) =  \frac{e^{ps_k}} { \sum_{k^\prime=i}^{j-1}{ e^{ps_{k^{\prime}}}}}. 
\end{equation*}

The training objective is to maximize the joint probability of all unlabeled production rules.
\begin{equation*}
    L_{\text{biaffine}} =  -\sum_{r \in {T_{ub}}} \log p(r: [i, j] \rightarrow [i, k] [k+1, j]) 
\end{equation*}

The decoding algorithm is the standard CKY algorithm, which we omit here. The biaffine model can be regarded as a 1st-order constituent model, with the probability of each phrase rule being modeled. However, unlike structured learning algorithms \cite{finkel2008crf,carreras2008tag}, which use a global score for each tree, our model learns each production rule probability individually. Such local learning has traditionally been found subjective to label bias \cite{lafferty2001conditional}. Our model relies on input representations solely for resolving this issue.


\subsection{Label generator}
\label{sec:encdec}

\begin{figure}[!t]
   \includegraphics[width=0.5\textwidth]{pics/encdec.pdf}
   \caption{Encoder-decoder structure for generating constituent spans.}
   \label{fig:encdec}
\end{figure}

We use the commonly used encoder-decoder framework \cite{cho2014properties,sutskever2014sequence} in  neural machine translation   to generate constituent labels and make unary rule decisions. Our encoder recursively composes vector representation of constituent spans for the unlabeled tree structure in a bottom-up style using tree-structured LSTM \cite{tai15treelstm,zhu15treelstm}. In particular, we use a lexicalized tree LSTM encoder \cite{zhiyang2016bitree} since there are no explicit lexical inputs for non-terminal spans. Using the output vectors from the encoder, the decoder generate constituent labels every span in the tree. Figure \ref{fig:encdec} shows the structure of our encoder-decoder model. We shows two label chains for the span $[4,4]$ and the span $[3, 3]$, respectively.  For the span $[4,4]$, there are collapsed unary rules S$\rightarrow$VP, our decoder firstly generates VP and then outputs S given that the previous label is VP. The decoding process continues until a ending symbol $<$/L$>$ is produced.   

\textbf{Lexicalized Tree-LSTM Encoder.} 
The lexicalized tree-LSTM encoder firstly propagates lexical information from two children spans to their parent using a lexical gate, then it produces the representation vectors of the parent span by composing the vectors of children spans using a binarizied tree-LSTM. 
Formally, the lexical vector $\mathbf{tx}[i,j]$ for the span $[i,j]$ with the partition point at $k$ is defined by:
\begin{equation*}
\small
    \begin{split}
        \mathbf{i}_{[i,j]}^{lex} &= \sigma ( \mathbf{W}_{l}^{lex} \mathbf{tx}{[i, k]} + \mathbf{W}_{r}^{lex} \mathbf{tx}{[k+1, j]} + \mathbf_{b}_{lex})\\
        \mathbf{tx}[i,j] &= \mathbf{i}_{[i,j]}^{lex} \odot \mathbf{tx}{[i, k]} + (\mathbf{1.0} - \mathbf{i}_{[i,j]}^{lex}) \odot \mathbf{tx}{[k+1, j]}, \\
    \end{split}
\end{equation*}
where $\mathbf{W}_{l}^{lex}$, $\mathbf{W}_{r}^{lex}$ and $\mathbf_{b}_{lex}$ are model parameters and $\odot$ is element-wise multiplication.  The lexical vector $\mathbf{tx}[i,i]$ for the leaf node $i$ is the concatenate of the output vectors of the BiLSTM encoder and the input representation $\mathbf{x}_{\textbf{input}}[i]$ (Equation \ref{eq:xinput}), as shown in Figure \ref{fig:encdec}.    

The output state vector $\mathbf{h}[i,j]$ of the span $[i,j]$  given by a binary tree LSTM encoder is, 
\begin{equation*}
\small
    \begin{split}
        \mathbf{i}_{[i,j]} =& \sigma (   \mathbf{W}_{xi} \mathbf{tx}_{[i,j]} +
         \mathbf{W}_{hi} ^ {l} \mathbf{h}_{[i,k]} + \mathbf{W}_{ci} ^ {l} \mathbf{c}_{[i,k]}  \\
        &  \mathbf{W}_{hi} ^ {r} \mathbf{h}_{[k+1,j]}  + \mathbf{W}_{ci} ^ {r} \mathbf{c}_{[k+1,j]} + \mathbf{b}_i )  \\
          \mathbf{f}_{[i,j]}^{l} =& \sigma (   \mathbf{W}_{xf}^{l} \mathbf{tx}_{[i,j]} +
         \mathbf{W}_{hf} ^ {ll} \mathbf{h}_{[i,k]} + \mathbf{W}_{cf} ^ {ll} \mathbf{c}_{[i,k]}  \\
        &  \mathbf{W}_{hf} ^ {lr} \mathbf{h}_{[k+1,j]} + \mathbf{W}_{cf} ^ {lr} \mathbf{c}_{[k+1,j]} + \mathbf{b}_f^{l} )  \\
         \mathbf{f}_{[i,j]}^{r} =& \sigma (   \mathbf{W}_{xf}^{r} \mathbf{tx}_{[i,j]} +
         \mathbf{W}_{hf} ^ {rl} \mathbf{h}_{[i,k]} + \mathbf{W}_{cf} ^ {rl} \mathbf{c}_{[i,k]}  \\
        &  \mathbf{W}_{hf} ^ {rr} \mathbf{h}_{[k+1,j]} + \mathbf{W}_{cf} ^ {rr} \mathbf{c}_{[k+1,j]} + \mathbf{b}_f^{r} )  \\
        \mathbf{g}_{[i,j]} =& \tanh (   \mathbf{W}_{xg} \mathbf{tx}_{[i,j]} +
         \mathbf{W}_{hg} ^ {l} \mathbf{h}_{[i,k]} + 
         \mathbf{W}_{hg} ^ {r} \mathbf{h}_{[k+1,j]}   + \mathbf{b}_g )  \\
         \mathbf{c}_{[i,j]}  =& \mathbf{f}_{[i,j]}^{l}  \odot  \mathbf{c}_{[i,k]}  +\mathbf{f}_{[i,j]}^{r}  \odot  \mathbf{c}_{[k+1,j]}+ \mathbf{i}_{[i,j]} \odot  \mathbf{g}_{[i,j]}\\
         \mathbf{o}_{[i,j]} =& \sigma (   \mathbf{W}_{xo} \mathbf{tx}_{[i,j]} +
         \mathbf{W}_{ho} ^ {l} \mathbf{h}_{[i,k]} + 
         \mathbf{W}_{ho} ^ {r} \mathbf{h}_{[k+1,j]}   \\
         & \mathbf{W}_{co} \mathbf{c}_{[i,j]}  + \mathbf{bt}_o)  \\
         \mathbf{h}_{[i,j]} = & \mathbf{o}_{[i,j]} \odot \tanh(\mathbf{c}_{[i,j]}).\\
    \end{split}
\end{equation*}

\textbf{Decoder.}  Suppose the constituent label chain for the span $[i,j]$ is ($\text{YL}_{[i,j]}^0, \text{YL}_{[i,j]}^1, \dots, \text{YL}_{[i,j]}^m$). The decoder for the span $[i,j]$ learns a conditional language model depending on the output vector $\mathbf{h}[i,j]$ from the tree LSTM encoder. Formally, the probability distribution of generating the label at time step $z$ is given by, 
\begin{equation*}
\begin{split}
    & P(\text{YL}_{[i,j]}^{z} | T_{ub}, \text{YL}_{[i,j]}^{z< m}) = \\
     &\text{softmax}\Big(g(\mathbf{h}[i,j], \mathbf{E}_{label} (\text{YL}_{[i,j]}^{z-1}), \mathbf{d}_{z-1})\Big), \\
\end{split}
\end{equation*}
where $\text{YL}_{[i,j]}^{z< m}$ is the decoding prefix, $\mathbf{d}_{z-1}$ is the state vector of the decoder LSTM and $\mathbf{E}_{label} (\text{YL}_{[i,j]}^{z-1})$ is the embedding of the previous output label.  

The training objective is to maximize the log-likelihood of the label generation distribution, 
\begin{equation*}
    \begin{split}
        \text{L}_{\text{label}}{[i,j]} &=  -\sum_{z=0}^{m} \log P(\text{YL}_{[i,j]}^{z} | T_{ub}, \text{YL}_{[i,j]}^{z< m}) \\
        \text{L}_{\text{label}} &= \sum_{[i,j] \in T_{ub} } \text{L}_{\text{label}}{[i,j]}. \\
    \end{split}
\end{equation*}

\subsection{Joint training.}

We jointly train the unlabeled parser and the label generator by minimize the overall loss 
\[
    L_{\text{total}} = L_{\text{parser}} + L_{\text{label}}  + \frac{\lambda}{2} ||\Theta||^2,
\]
where $\lambda$ is a regularization hyper-parameter. We set $L_{\text{parser}}=L_{\text{binary}}$ and $L_{\text{parser}}=L_{\text{biaffine}}$ when using the binary classification model and the biaffine model, respectively. 

==> part/model1.tex <==
\section{Model}
\begin{figure*}[t]
\begin{subfigure}[b]{0.5\textwidth}
\centering
   \includegraphics[width=0.7\textwidth]{pics/spanclas2.pdf}
   \caption{BiLSTM based constituent span classifier.}
   \label{fig:spanclas}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\includegraphics[width=\textwidth]{pics/treeb.pdf}
\caption{Unlabeled binarized parse tree.}
\label{fig:binarized}
\end{subfigure}
\begin{subfigure}[b]{0.55\textwidth}
\centering
\includegraphics[width=\textwidth]{pics/treec.pdf}
\caption{Label generator. \textbf{NP*} is an intermediate constituent label. $<$/L$>$ is an ending marker.}
\label{fig:binlabeltree}
\end{subfigure}
\begin{subfigure}[b]{0.4\textwidth}
    \centering
\includegraphics[width=\textwidth]{pics/treed.pdf}
\caption{Final example parse tree.}
\label{fig:fulltree}
\end{subfigure}
\caption{An overview workflow of our chart-based neural greedy constituent parser for processing the sentence ``The stock price keeps falling''. We annotate every non-terminal span with its covered span range. Figure \ref{fig:spanclas} shows constituent span classifiers making 0/1 decisions for all possible spans. Based on the local classification probabilities, we obtain an unlabeled binarized parse tree (Figure \ref{fig:binarized}) using binary CKY parsing algorithms. We then hierarchically generate labels for each span (Figure \ref{fig:binlabeltree}) using encoder-decoder models. Figure \ref{fig:fulltree} shows the final output parse tree after debinarization.}
\label{fig:all}
\end{figure*}

Our models consist of an unlabeled binarized tree parser and a label generator. 
Figure \ref{fig:all} shows a running example of our parsing model.  
The unlabeled parser (Figure \ref{fig:spanclas}, \ref{fig:binarized}) learns an unlabeled parse tree using simple BiLSTM encoders.  The label generator (Figure \ref{fig:binlabeltree}, \ref{fig:fulltree})  predicts constituent labels for each span in the unlabeled tree using encoder-decoder models. 

For a sentence $S$, the unlabeled parser employs classification models to describe the probability $P([i, j] \rightarrow [i, k] [k+1, j]|S)$ for the span production rule that the span $[i, j]$ is composed by two children spans $[i, k]$ and $[k+1, j]$ where $i\leq k < j$.  
We then use the CKY algorithm to derive unlabeled binarized parse trees based on span production probabilities,  

In particular, we design two different classification models for unlabeled parsing: the \textbf{span model} (Section \ref{sec:binary}) and the \textbf{rule model} (Section \ref{sec:biaffine}). 
The span model identifies the probability of an arbitrary span being a constituent span. 
For example, the span $[1,2]$ in Figure \ref{fig:spanclas} belongs to the correct parse tree (Figure \ref{fig:fulltree}). Ideally, our model assigns a high probability to this span.  
In contrast, the span $[0,3]$ is not a valid constituent span and our model labels it with 0. 
Different from the span  model,  the rule model directly considers the probability of the splitting point $k$ ($i\leq k < j$) for a span $[i,j]$.  For example, in Figure \ref{fig:spanclas}, $k=0$ is a better partition point for span $[0, 2]$ than $k=1$. Therefore, the rule model assigns high probability to the rule $[0, 2] \rightarrow [0, 0] [1, 2]$ instead of the rule $[0, 2] \rightarrow [0, 1] [2, 2]$.  

The label generator adopts an encoder-decoder \cite{cho2014properties,sutskever2014sequence} framework to encode a binarized unlabeled tree and to decode constituent labels for every span. 
The encoder is a binary tree-LSTM encoder \cite{tai15treelstm,zhu15treelstm} which composes the representation vectors for tree nodes in a bottom-up style. 
Based on the representation vector of a constituent span, the decoder generates chains of constituent labels. For example, the decoder outputs ``VP $\rightarrow$S$ \rightarrow$ $<$/L$>$'' for the span [4, 4]  and ``NP$\rightarrow$ $<$/L$>$'' for the span [0,2] in Figure \ref{fig:binlabeltree} where $<$/L$>$ is a stopping symbol. 
\subsection{Span Model}
\label{sec:binary}
 Given an unlabeled binarized tree $T_{ub}$ for the sentence $S$, $S= w_0, w_1 \dots w_{n-1}$,  the span model trains a neural network model $P(Y_{[i,j]}|S, \Theta)$ to distinguish  constituent spans from  non-constituent spans, where $0 \leq i \leq n-2$, $ 1 \leq j < n$, $i < j$, $Y_{[i, j]} =1 $ indicates the span [i, j] is a constituent span ($[i, j] \in T_{ub}$), and  $Y_{[i, j]} =0 $ for otherwise, $\Theta$ are model parameters.  We do not model spans with length 1 since the span $[i, i]$ always belongs to $T_{ub}$. 


\textbf{Network Structure.} Figure \ref{fig:binclas} shows the neural network structures for the binary classification model. In the bottom, a bidirectional LSTM layer encodes the input sentence to extract non-local features. In particular, we append a starting symbol $<$s$>$ and an ending symbol $<$/s$>$ to the left-to-right LSTM and the right-to-left LSTM, respectively.   We denote the output hidden vectors of the left-to-right LSTM and the right-to-left LSTM  for $w_0, w_1, \dots, w_{n-1}$ 
is $\mathbf{f}_1, \mathbf{f}_2, \dots, \mathbf{f}_n$ and $\mathbf{r}_0, \mathbf{r}_1, \dots, \mathbf{r}_{n-1}$, respectively.  
We obtain the representation vector $\mathbf{v}[i, j]$ of the span $[i, j]$ by simply concatenating the bidirectional output vectors at the input word $i$ and the input word $j$,
\begin{equation}
\small
\mathbf{v}[i,j]=[\mathbf{f}_{i+1};\mathbf{r}_{i}; \mathbf{f}_{j+1}; \mathbf{r}_{j}].
\label{eq:v}
\end{equation}
We then pass $\mathbf{v}[i, j]$ through a nonlinear transformation and get the probability distribution 
$P(Y_{[i,j]}|S, \Theta)$ by
\begin{equation}
\label{eq:binaryp}
\small
        \mathbf{o}[i,j] = \tanh (\mathbf{W}_o \mathbf{v}[i,j] + \mathbf{b}_o),\ \  
        \mathbf{u}[i,j] = \mathbf{W}_u \mathbf{o}[i,j] + \mathbf{b}_u, \ \ 
        P(Y_{[i,j]}|S, \Theta) = \text{softmax}(\mathbf{u}[i,j]), 
\end{equation}
where $\mathbf{W}_o, \mathbf{b}_o, \mathbf{W}_u$ and $\mathbf{b}_u$ are model parameters. 

\textbf{Input Representation.} For the parsing tasks, the input sentence usually contains words and part-of-speech (POS) tags, we combine them together to obtain the input representation vectors.  Given a word $w$, its corresponding characters $c_0,\dots, c_{|w|-1}$ and POS tag $t$, first, we get the word embedding $\mathbf{E}_{word}^w$, character embeddings $\mathbf{E}_{char}^{c_0},\dots, \mathbf{E}_{char}^{c_{|w|-1}}$, and POS tag embedding $\mathbf{E}_{pos}^t$ using lookup operations. Then we use a bidirectional LSTM to extract character-level features. Suppose the output vectors of the last step of the left-to-right and right-to-left LSTMs are $\mathbf{h}_{char}^f$ and $\mathbf{h}_{char}^r$, respectively.  The final input vector $\mathbf{x}_{input}$ is given by 
\begin{equation}
\small
        \mathbf{x}_{char} = \tanh (\mathbf{W}_{char}^f \mathbf{h}_{char}^f +  \mathbf{W}_{char}^r \mathbf{h}_{char}^r + \mathbf{b}_{char} ),  \ \ 
        \mathbf{x}_{input} = [ \mathbf{E}_{word}^w + \mathbf{x}_{char};  \mathbf{E}_{pos}^t],
\label{eq:xinput}
\end{equation}
where $\mathbf{W}_{char}^f$, $\mathbf{W}_{char}^r$ and $\mathbf{b}_{char}$ are model parameters. 
\newcite{wang2015char} demonstrated that the input representation vector $\mathbf{E}_{word}^w + \mathbf{x}_{char}$ obtained the-state-of-the-art POS tagging accuracy.  Inspired by their experiments, we design this network to combine words, characters and POS tags as input representations for constituent parsing.

\textbf{Training objective.} The training objective is to maximize the probabilities of $P(Y_{[i,j]}=1|S, \Theta)$ for spans $[i,j] \in T_{ub}$ and minimize the probabilities of $P(Y_{[i,j]}=1|S, \Theta)$ for spans $[i,j] \notin T_{ub}$ at the same time. 
Formally, the training loss for binary span classification $L_{\text{span}}$ is given by
\begin{equation}
\small
    L_{\text{binary}} = -\sum_{[i,j] \in T_{ub}}{ \log P(Y_{[i,j]} = 1 | S, \Theta)}  -\sum_{[i,j] \notin T_{ub}}{ \log P(Y_{[i,j]} = 0 |S, \Theta)}, \ 
    (0 \leq i \leq n-2, 1 \leq j < n, i < j)
\label{eq:binloss}
\end{equation}
For a sentence with length $n$, there are $\frac{ n (n -1) } {2}$ terms in total in Eq \ref{eq:binloss}. 


\begin{figure*}[!t]
\begin{subfigure}[b]{0.48\textwidth}
   \includegraphics[width=\textwidth]{pics/binaryclas.pdf}
   \caption{Span model.  \vspace{-1em} }
   \label{fig:binclas}
\end{subfigure}
\begin{subfigure}[b]{0.48\textwidth}
   \includegraphics[width=\textwidth]{pics/biaffinescore.pdf}
   \caption{Rule model.  \vspace{-1em} }
   \label{fig:biaffine}
\end{subfigure}
\caption{Two different models for constituent span classification using BiLSTM encoders. \vspace{-1em} }
\label{fig:model}
\end{figure*}



\textbf{Neural CKY algorithm.} The unlabeled production probability for the rule $r:[i, j]\rightarrow[i, k][k+1, j]$  given by the binary classification model is,  
\begin{equation*}
\small
P(r | S, \Theta) = P( Y_{[i, k]} = 1 |S, \Theta )P( Y_{[k+1, j]} = 1 |S, \Theta).
\end{equation*}
 During decoding, we find the optimal parse tree $T_{ub}^{*}$ using the CKY algorithm. Note that our CKY algorithm is different from the standard CKY algorithm mainly in that there is no phrase rule probabilities $P([i, j] \rightarrow [i, k][k+1, j]|S, \Theta)$ being involved. Hence our model can be regarded as a 0-order constituent tree model, which is the most {\it local}. All structural relations in a constituent tree must be implicitly captured by the BiLSTM encoder over the sentence alone. 

\textbf{Multi-class Span Classification Model.} The previous model preforms binary classifications to identify constituent spans. In this way,  the classification model  only captures the existence of constituent labels but does not leverage the  constituent label type information. In order to incorporate the syntactic label information into the span model, we also propose a multi-class span classification model $P(Y_{[i,j]}=c|S, \Theta)$ to describe the probability that $c$ is a constituent label for span $[i,j]$.  The network structure is almost the same as the binary span classification model except the last layer.  For the last layer, suppose we already obtain $\mathbf{o}_{[i,j]}$ in Eq \ref{eq:binaryp},  $P(Y_{[i,j]}=c|S, \Theta)$ is then calculated by,
\begin{equation}
\label{eq:multip}
        \mathbf{m}[i,j] = \mathbf{W}_m \mathbf{o}[i,j] + \mathbf{b}_m, \
        P(Y_{[i,j]}=c|S, \Theta) = \text{softmax}(\mathbf{m}[i,j]).
\end{equation}
Here $\mathbf{W}_m, \mathbf{b}_m, \mathbf{W}_m$ and $\mathbf{b}_m$ are model parameters. The training objective is,
\begin{equation}
\small
\begin{split}
    L_{\text{multi}} = -\sum_{[i,j] \in T_{ub}}\sum_{c \in [i,j], c\neq \text{$<$}/L\text{$>$} }{ \log &P(Y_{[i,j]} = c | S, \Theta)} 
    -\sum_{[i,j] \notin T_{ub}}{ \log P(Y_{[i,j]} = \text{$<$}/L\text{$>$} |S, \Theta)}, \\
    & (0 \leq i \leq n-2, 1 \leq j < n, i < j)\\
\end{split}
\label{eq:mutiloss}
\end{equation}
Note that there is an additional sum inside the first term in Eq \ref{eq:mutiloss}, which is different from the first term in Eq \ref{eq:binloss}. This is to say that we treat all constituent labels equally of a unary chain. For example, there is a unary chain S$\rightarrow$VP in span [4,4]. For this span, we hypothesize that both these two labels are possible answers for this span and pay equal attentions to $VP$ and $S$ during training. For the second term in Eq \ref{eq:mutiloss}, we maximize the probability of the ending label for non-constituent spans. 

For decoding, we transform the multi-class probability distribution into a binary probability distribution by using,
\begin{equation*}
\small
P(Y_{[i,j]}=1|S, \Theta) = \sum_{c, c\neq \text{$<$}/L\text{$>$} }{ P(Y_{[i,j]} = c | S, \Theta)},    \ \ 
     P(Y_{[i,j]}=0|S, \Theta) = P(Y_{[i,j]}=\text{$<$}/L\text{$>$} |S, \Theta)
\label{eq:transform}
\end{equation*}
In this way, the probability of a span being a constituent span takes all possible syntactic labels into considerations. 

\subsection{Rule Model}
\label{sec:biaffine}

The rule model directly calculates the probabilities of all possible splitting points $k$ ($ i\leq k < j)$ for the span $[i, j]$. Suppose the partition score of splitting point $k$ is $ps_k$. The unlabeled production probability for the rule $r:[i, j]\rightarrow[i, k][k+1, j]$ is given by a softmax distribution, 
\begin{equation*}
\small
 P([i, j] \rightarrow [i, k] [k+1, j]|S, \Theta) =  \frac{e^{ps_k}} { \sum_{k^\prime=i}^{j-1}{ e^{ps_{k^{\prime}}}}}. 
\end{equation*}
The training objective is to maximize the joint probability of all unlabeled production rules.
\begin{equation*}
\small
L_{\text{rule}} =  -\sum_{r \in {T_{ub}}} \log P(r: [i, j] \rightarrow [i, k] [k+1, j]|S, \Theta)
\end{equation*}

The decoding algorithm is the standard CKY algorithm, which we omit here. The rule model can be regarded as a 1st-order constituent model, with the probability of each phrase rule being modeled. However, unlike structured learning algorithms \cite{finkel2008crf,carreras2008tag}, which use a global score for each tree, our model learns each production rule probability individually. Such local learning has traditionally been found subjective to label bias \cite{lafferty2001conditional}. Our model relies on input representations solely for resolving this issue.

\textbf{Span Representation.} Figure \ref{fig:biaffine} shows one possible network architecture for the rule model by taking the partition point $k=1$ for the span $[1, 3]$ as an example. 
The BiLSTM encoder layer in the bottom is the same as that in the previous span classification model. We obtain the span representation vectors using difference vectors \cite{wang2016graph,james2016span}. Formally, the span representation vector $\mathbf{sr}[i, j]$ is given by,
\begin{equation}
\small
\mathbf{s}[i, j]=[\mathbf{f}_{j+1} - \mathbf{f}_{i}; \mathbf{r}_{i} - \mathbf{r}_{j+1}],  \ \ 
\mathbf{sr}[i, j]=[ \mathbf{s}[0, i-1]; \mathbf{s}[i, j]; \mathbf{s}[j+1, n-1]]. 
    \label{eq:spanrep}
\end{equation}
We first combine the difference vectors $(\mathbf{f}_{j+1} - \mathbf{f}_{i})$ and $(\mathbf{r}_{i} - \mathbf{r}_{j+1})$ to get a simple span representation vector $\mathbf{s}[i, j]$.  
In order to take more contextual information such as $\mathbf{f}_p$ where $p>j+1$ and $\mathbf{r}_q$ where $q<i$, we concatenate $\mathbf{s}[0, i-1]$,  $\mathbf{s}[i, j]$, and $\mathbf{s}[j+1, n-1]$ together to produce the final span representation vector $\mathbf{sr}[i, j]$.  We then transform $\mathbf{sr}[i,j]$ to get an output vector $\mathbf{r}[i,j]$ using an activation function $\phi$ to exploit the representation power of nonlinear span features,
\begin{equation}
\small
\label{eq:r}
         \mathbf{r}[i,j] = \phi (\mathbf{W}_r^{M} \mathbf{sr}[i,j] + \mathbf{b}_r^{M}), 
\end{equation}
where $\mathbf{W}_r^{M}$ and $\mathbf{b}_r^{M}$ and model parameters, and $M$ is a parameter set index. We use separate parameters for the nonlinear transforming layer. $M\in \{P, L, R\}$ are for the parent span $[i, j]$, the left child span $[i,k]$ and the right child span $[k+1, j]$, respectively.  

After obtaining the span representation vectors, we use these vectors to calculate the partition score $ps_k$. In particular, we investigate two scoring methods.  

\textbf{Linear Model.} In the linear model, the partition score is calculated by a linear affine transformation. For the splitting point $k$, 
\begin{equation*}
\small
    ps_k = \mathbf{w}_{ll, k}^T \mathbf{r}[i, k] + \mathbf{w}_{lr, k}^T \mathbf{r}[k+1, j] + {b}_{ll,k}
\end{equation*}
where $\mathbf{w}_{ll, k}^T$ and $\mathbf{w}_{ll, k}^T$ are two vectors, and ${b}_{ll,k}$ is a size 1 parameter. 

\textbf{Biaffine model.} Since the possible splitting points for spans are varied with the length of span, we also try a biaffine scoring model (as shown in Figure \ref{fig:biaffine}) which is good at handling variable-sized classification problems \cite{Dozat2016biaffine,ma2017neural}. The biaffine model  produces the score ${lps}_k$ between the parent span $[i,j]$ and the left child span $[i, k]$ using a biaffine scorer
\begin{equation}
\small
         {lps}_k = (\mathbf{r}[i,j] \oplus 1)^{T} \mathbf{W}_{pl} (\mathbf{r}[i,k] \oplus 1) 
\end{equation}
where $\mathbf{W}_{pl}$ is model parameters. 
Similarly, we calculate the score ${rps}_k$ between the parent span $[i,j]$ and the right child span $[k+1, j]$ using $\mathbf{W}_{pr}$ and $\mathbf{b}_{pr}$ as parameters.  The overall partition score ${ps}_k$ is therefore given by 
\[
{ps}_k  = {lps}_k + {rps}_k.
\]
\iffalse
\textbf{Triaffine model.} The biaffine model captures richer interactions between two span vectors than the linear model. We continue increase the interactions among span vectors and model the interaction of three span vectors using a low-rank tensor scorer. We name this model as triaffine model. In this model, the elements in the parent span vector $\mathbf{r}[i,j]$ can jointly interact with every element in two children span vectors $\mathbf{r}[i,k]$ and $\mathbf{r}[k+1,j]$. One way to connect three vector together is to use tensor product. However, directly using tensor product is very expensive. We thus turn to an low-rank based approximate method used in \cite{lei-barzilay-jaakkola:2015:EMNLP}. Formally, the partition score is given by,
\begin{equation*}
\small
        \mathbf{z} = \mathbf{O}^T  \Big(\mathbf{P}(\mathbf{r}[i,j]\oplus 1)\Big) \Big(\mathbf{Q}(\mathbf{r}[i,k]\oplus 1)\Big) 
         \Big(\mathbf{R}(\mathbf{r}[k+1,j]\oplus 1)\Big), \ \ 
        ps_k = \mathbf{w}_{z, k}^T \mathbf{z} + b_{z, k} 
\end{equation*}
Here $\mathbf{O}$, $\mathbf{P}$, $\mathbf{Q}$, $\mathbf{R}$, $\mathbf{w}_{z, k}$ and $b_{z, k}$ are model parameters. The biaffine scorer can be regared as a degrade version of triaffine scorer. And similarly, the linear scorer is a specical version of the triaffine model. 
\fi
\subsection{Label generator}
\label{sec:encdec}

\begin{figure}[!t]
\centering
   \includegraphics[width=0.5\textwidth]{pics/encdec.pdf}
   \caption{Encoder-decoder structure for generating constituent spans. \vspace{-1.5em}}
   \label{fig:encdec}
\end{figure}

We adopt the commonly used encoder-decoder framework \cite{cho2014properties,sutskever2014sequence} in  neural machine translation   to generate constituent labels and to make unary rule decisions. Our encoder recursively composes vector representation of constituent spans for the unlabeled tree structure in a bottom-up style using tree-structured LSTM \cite{tai15treelstm,zhu15treelstm}. In particular, we use a lexicalized tree LSTM encoder \cite{zhiyang2016bitree} since there are no explicit lexical inputs for non-terminal spans. Using the output vectors from the encoder, the decoder generates constituent labels for every span in the tree. Figure \ref{fig:encdec} shows the structure of our encoder-decoder model. We show two label chains for the span $[4,4]$ and the span $[3, 4]$, respectively.  For the span $[4,4]$, there are collapsed unary rules S$\rightarrow$VP, our decoder first generates VP and then outputs $S$ given that the previous label is VP. The decoding process continues until a ending symbol $<$/L$>$ is produced.   

\textbf{Lexicalized Tree-LSTM Encoder.} 
The lexicalized tree-LSTM encoder first propagates lexical information from two children spans to their parent using a lexical gate, then it produces the representation vectors of the parent span by composing the vectors of children spans using a binarized tree-LSTM. 
Formally, the lexical vector $\mathbf{tx}[i,j]$ for the span $[i,j]$ with the partition point at $k$ is defined by:
\begin{equation*}
\small
    \begin{split}
        \mathbf{i}_{[i,j]}^{lex} &= \sigma ( \mathbf{W}_{l}^{lex} \mathbf{tx}{[i, k]} + \mathbf{W}_{r}^{lex} \mathbf{tx}{[k+1, j]} +    \mathbf{W}_{lh}^{lex}\mathbf{h}_{[i,k]} + \mathbf{W}_{rh}^{lex}\mathbf{h}_{[k+1,j]} +  \mathbf{b}_{lex})\\
        \mathbf{tx}[i,j] &= \mathbf{i}_{[i,j]}^{lex} \odot \mathbf{tx}{[i, k]} + (\mathbf{1.0} - \mathbf{i}_{[i,j]}^{lex}) \odot \mathbf{tx}{[k+1, j]}, \\
    \end{split}
\end{equation*}
where $\mathbf{W}_{l}^{lex}$, $\mathbf{W}_{r}^{lex}$ and $\mathbf{b}_{lex}$ are model parameters and $\odot$ is element-wise multiplication.  The lexical vector $\mathbf{tx}[i,i]$ for the leaf node $i$ is the concatenate of the output vectors of the BiLSTM encoder and the input representation $\mathbf{x}_{\textbf{input}}[i]$ (Eq \ref{eq:xinput}), as shown in Figure \ref{fig:encdec}.    

The output state vector $\mathbf{h}[i,j]$ of the span $[i,j]$  given by a binary tree LSTM encoder is, 
\begin{equation*}
\small
    \begin{split}
        \mathbf{i}_{[i,j]} =& \sigma (   \mathbf{W}_{xi} \mathbf{tx}_{[i,j]} +
         \mathbf{W}_{hi} ^ {l} \mathbf{h}_{[i,k]} + \mathbf{W}_{ci} ^ {l} \mathbf{c}_{[i,k]} + 
          \mathbf{W}_{hi} ^ {r} \mathbf{h}_{[k+1,j]}  + \mathbf{W}_{ci} ^ {r} \mathbf{c}_{[k+1,j]} + \mathbf{b}_i )  \\
          \mathbf{f}_{[i,j]}^{l} =& \sigma (   \mathbf{W}_{xf}^{l} \mathbf{tx}_{[i,j]} +
         \mathbf{W}_{hf} ^ {ll} \mathbf{h}_{[i,k]} + \mathbf{W}_{cf} ^ {ll} \mathbf{c}_{[i,k]}  + 
          \mathbf{W}_{hf} ^ {lr} \mathbf{h}_{[k+1,j]} + \mathbf{W}_{cf} ^ {lr} \mathbf{c}_{[k+1,j]} + \mathbf{b}_f^{l} )  \\
         \mathbf{f}_{[i,j]}^{r} =& \sigma (   \mathbf{W}_{xf}^{r} \mathbf{tx}_{[i,j]} +
         \mathbf{W}_{hf} ^ {rl} \mathbf{h}_{[i,k]} + \mathbf{W}_{cf} ^ {rl} \mathbf{c}_{[i,k]} +
         \mathbf{W}_{hf} ^ {rr} \mathbf{h}_{[k+1,j]} + \mathbf{W}_{cf} ^ {rr} \mathbf{c}_{[k+1,j]} + \mathbf{b}_f^{r} )  \\
        \mathbf{g}_{[i,j]} =&\tanh (   \mathbf{W}_{xg} \mathbf{tx}_{[i,j]} + 
         \mathbf{W}_{hg} ^ {l} \mathbf{h}_{[i,k]} + 
          \mathbf{W}_{hg} ^ {r} \mathbf{h}_{[k+1,j]}   + \mathbf{b}_g )  \\
         \mathbf{c}_{[i,j]}  =& \mathbf{f}_{[i,j]}^{l}  \odot  \mathbf{c}_{[i,k]}  +\mathbf{f}_{[i,j]}^{r}  \odot  \mathbf{c}_{[k+1,j]}+ \mathbf{i}_{[i,j]} \odot  \mathbf{g}_{[i,j]}\\
         \mathbf{o}_{[i,j]} =& \sigma (   \mathbf{W}_{xo} \mathbf{tx}_{[i,j]} +
         \mathbf{W}_{ho} ^ {l} \mathbf{h}_{[i,k]} + 
         \mathbf{W}_{ho} ^ {r} \mathbf{h}_{[k+1,j]}   +
          \mathbf{W}_{co} \mathbf{c}_{[i,j]}  + \mathbf{bt}_o)  \\
         \mathbf{h}_{[i,j]} = & \mathbf{o}_{[i,j]} \odot \tanh(\mathbf{c}_{[i,j]}).\\
    \end{split}
\end{equation*}

\textbf{Decoder.}  Suppose the constituent label chain for the span $[i,j]$ is ($\text{YL}_{[i,j]}^0, \text{YL}_{[i,j]}^1, \dots, \text{YL}_{[i,j]}^m$). The decoder for the span $[i,j]$ learns a conditional language model depending on the output vector $\mathbf{h}[i,j]$ from the tree LSTM encoder. Formally, the probability distribution of generating the label at time step $z$ is given by, 
\begin{equation*}
\small
    P(\text{YL}_{[i,j]}^{z} | T_{ub}, \text{YL}_{[i,j]}^{z< m}) = 
     \text{softmax}\Big(g(\mathbf{h}[i,j], \mathbf{E}_{label} (\text{YL}_{[i,j]}^{z-1}), \mathbf{d}_{z-1})\Big), 
\end{equation*}
where $\text{YL}_{[i,j]}^{z< m}$ is the decoding prefix, $\mathbf{d}_{z-1}$ is the state vector of the decoder LSTM and $\mathbf{E}_{label} (\text{YL}_{[i,j]}^{z-1})$ is the embedding of the previous output label.  

The training objective is to maximize the log-likelihood of the label generation distribution, 
\begin{equation*}
\small
        \text{L}_{\text{label}}{[i,j]} =  -\sum_{z=0}^{m} \log P(\text{YL}_{[i,j]}^{z} | T_{ub}, \text{YL}_{[i,j]}^{z< m}), \ \ 
        \text{L}_{\text{label}} = \sum_{[i,j] \in T_{ub} } \text{L}_{\text{label}}{[i,j]}. 
\end{equation*}

\subsection{Joint training}
The unlabeled parser and the label generator share parts of network components, such as word embeddings, char embeddings, POS embedding and the BiLSTM encoding layer. 
We jointly train the unlabeled parser and the label generator by minimizing the overall loss 
\[
    L_{\text{total}} = L_{\text{parser}} + L_{\text{label}}  + \frac{\lambda}{2} ||\Theta||^2,
\]
where $\lambda$ is a regularization hyper-parameter. We set $L_{\text{parser}}=L_{\text{binary}}$ or $L_{\text{parser}}=L_{\text{multi}}$ and $L_{\text{parser}}=L_{\text{rule}}$ when using the binary classification model and the biaffine model, respectively. 
